Evaluating Subtitle Segmentation for End-to-end Generation Systems

Subtitles appear on screen as short pieces of text, segmented based on formal constraints (length) and syntactic/semantic criteria. Subtitle segmentation can be evaluated with sequence segmentation metrics against a human reference. However, standard segmentation metrics cannot be applied when systems generate outputs different than the reference, e.g. with end-to-end subtitling systems. In this paper, we study ways to conduct reference-based evaluations of segmentation accuracy irrespective of the textual content. We first conduct a systematic analysis of existing metrics for evaluating subtitle segmentation. We then introduce $Sigma$, a new Subtitle Segmentation Score derived from an approximate upper-bound of BLEU on segmentation boundaries, which allows us to disentangle the effect of good segmentation from text quality. To compare $Sigma$ with existing metrics, we further propose a boundary projection method from imperfect hypotheses to the true reference. Results show that all metrics are able to reward high quality output but for similar outputs system ranking depends on each metric's sensitivity to error type. Our thorough analyses suggest $Sigma$ is a promising segmentation candidate but its reliability over other segmentation metrics remains to be validated through correlations with human judgements.

==> bleus.tex <==
\begin{figure*}[t]
  \centering
  \begin{tabular}{l p{0.9\textwidth}}
    \hline 
    REF &  the car has just left Paris \eol for its destination London \eos where it will arrive next sunday \eol if all goes well . \eob \\
    HYP & the car has just left Paris \eol for his destination : London \eos where he arrive \eol  next sunday if \eol all goes well . \eob \\
    \hline
  \end{tabular}
  
  \vspace{\baselineskip}
  
  The bigram ``\textcolor{blue}{left Paris}'' and trigram ``\textcolor{blue}{all goes well}'' match both for \bleunb{} and \bleubr; the bigram ``\textcolor{blue}{London \eol}'' and the trigram ``\textcolor{blue}{Paris \eol for}'' match for \bleubr{} but not for \bleunb{}; conversely the bigram ``if all'' and trigram ``arrive next sunday'' match for \bleunb, but not for \bleubr.
  \caption{Comparing \bleunb{} and \bleubr{}}
  \label{fig:bleubr}
\end{figure*}

In spite of its flaws, \bleunb{} remains the go-to metrics for MT papers and for studies about subtitling. 
\bleunb{} computes a global evaluation of the content match between the reference and the hypothesis text, averaging modifed precision scores for n-gram of various size (typically from $n=1$ to $n=4$). As explained above, for perfect output text (\bleunb{}=100) \bleubr{} deliver scores that correlate well with precision/recall/F1 metrics, with the added benefit of yielding a global aggregate value taking into account all types of error (ins, del, sub). The question we now turn to is the usefulness of \bleubr \emph{for imperfect texts}. What we would like to have is to independently evaluate progress in content prediction (with BLEU) and progress in segmentation prediction. Can \bleubr{}, used in previous work, play that role ?

We first acknowledge that for fixed \bleunb{}, \bleubr{} actually ranks segmentation from good to bad, yet is slightly unbalanced towards prefering additions over deletions and replacements, then shifts; shifts  of different values are treated almost equally. Segmentation errors yield \bleubr{} range that can go from simple to double in absolute terms; even for small amounts of noise, we see that BLEU can drop by approximately 10 to 20\%. 

Which is higher ? For \bleunb{}$=$100 we cannot do better; as \bleunb{} goes down, the easier it is to observe \bleubr{} values greater than \bleunb{} \footnote{\textcolor{red}{only 2 values for a.20 - \bleunb{}=58.59; 7 values for a.30 - \bleunb{}=42.93; 11 values for a.40 \bleunb{}=29.33.}}, which means that the (absolute or relative) difference between the two cannot be a proper signal of segmentation quality alone. So the simple line of reasoning that would just see in \bleunb{} > \bleubr{} a sign of a good segmentation is correct, but the intensity of this signal can not be realistically assessed from these two measures alone.

How can we have \bleunb{} $<$ \bleubr{} ? This is because the latter is based on longer sentences, which means more n-grams to match. As predicting the right number and types of tags is generally easier than for content words, \bleubr{} usally has a higher 1g precision, which can have an effect on the higher-order scores.\footnote{Almost all simulations have 1g precisions higher for \bleubr{} than for \bleunb{}.}.
\fyTodo{Do we this is on actual data?}

This suggests viewing the differences between the two scores as resulting from the matches obtained for $n$-grams containing a tag (henceforth \emph{$n$-tagrams}), and hints at separatly computing two scores: \bleunb{} on the one hand, and \bleuem{} which only computes precision scores wrt.\ n-tagram: unigram precisions would be just for segmentation tags; bigram precisions for 2-tagrams such as ``w \gtag{}'' or ``\gtag{} w'' etc.\footnote{An approach investigated by E. Michon, personal communication with the authors.} \bleuem{} however remains highly correlated with \bleunb{}: this is because $n$-tagram matches for this metric directly depend on the level of $n-1$-grams for \bleunb. For instance, ``w$_1$ w$_2$ \gtag'' can only be correct if ``w$_1$ w$_2$'' is also a match, implying that the $n$-gram scores imply an upper bound on the possible $n+1$-tagram matches.
 
5. Notations: we denote $p_1, p_2, p_3, p_4$ respectively the 1g, 2g, 3g and 4g modified precisions computed by \bleunb{}, and $\alpha$ the proportion of the number of break tags to the number of regular tokens, and ${p'}_1, \dots{} {p'}_4$ the corresponding quantities for \bleubr{}. Under the assumption that break tags are mostly correct, the expected number of 1-grams in a text of $l$ words augmented with tags is just $p_u \times l + \alpha \times{} l$, yielding ${p'}_u = \frac{1 + \alpha}{p_u + \alpha}$. For higher order n-grams, the exact computation is more involved, but a simple upper bound is defined as follows:
$$
{p'}_{n} \le \frac{p_{n} +  \alpha \times p_{n-1} }{1+\alpha}.
$$
This holds because we assume that all (a) correct $n$-grams matching for \bleunb{} also match for \bleubr{}; (b) each $n-1$ gram
matched for \bleunb{} yields (at most) one new n-tagrams (in theory it might create two: one with the tag on the right, one with a tag on the left, but this would imply very short lines and does hardly appear in our references); (c) the text length is sufficiently long so that we can make the approximation $\frac{l}{l+1} \approx{} 1$. We readily derive an upper bound \bleubr$^+$ of \bleubr{} that we can compute from \bleunb{}. This value can be used as a proxy to the best achievable \bleubr{}s for a given \bleunb{}: denoting $S$ the ratio $S = \frac{\text{\bleubr}}{\text{\bleubr}^+}$, we have that values close to $1$ would denote good segmentations, while values close to $0$ denote bad segmentations \emph{irrespective of the value of} \bleunb. We illustrate this on Figure~\ref{} where we plot XXXX.



==> comments.tex <==
 %We have noticed that end-to-end systems have do not over- or under-generate boundaries (e.g. the outputs of the systems in Section~\ref{exp3} have less than 10\% difference in the number of boundaries compared to the reference). WHY EQUAL WEIGHT ADD,DEL,REP? 
%With shifts, the affected subtitles become longer or shorter, which will lead to the reading speed being too high for some subtitles, while others will unnecessarily linger on the screen, resulting in re-reading effects. Despite this, the length conformity was always kept above 86\% regardless of the size and percentage of shift, which means that shifting does not lead to overly long subtitles. Deletions imply subtitles with a correct reading speed and segmentation according to linguistic units but too long to fit the screen. This may result in viewers missing a part of the subtitle. On the contrary, additions lead to shorter and faster subtitles, while the added boundaries may also break linguistic units. As a result, the processing difficulty of subtitles will be higher. Replacements do not affect the linguistic units, but simply lead to a different distribution of the subtitles. The critical error that could result is multiple \eol{} which would render invalid displays of more than 2 lines.  However, we have noticed that this rarely happens in end-to-end systems. 
%For this reason, we wish to penalise them less than other types of noise and all metrics seem to achieve this. 
